Clustering Internet Memes Through Template Matching and Multi-Dimensional Similarity

Meme clustering is critical for toxicity detection, virality modeling, and typing, but it has received little attention in previous research. Clustering similar Internet memes is challenging due to their multimodality, cultural context, and adaptability. Existing approaches rely on databases, overlook semantics, and struggle to handle diverse dimensions of similarity. This paper introduces a novel method that uses template-based matching with multi-dimensional similarity features, thus eliminating the need for predefined databases and supporting adaptive matching. Memes are clustered using local and global features across similarity categories such as form, visual content, text, and identity. Our combined approach outperforms existing clustering methods, producing more consistent and coherent clusters, while similarity-based feature sets enable adaptability and align with human intuition. We make all supporting code publicly available to support subsequent research.

==> intro.tex <==

% Background

% Memes are a crucial communication tool on social media, condensing complex ideas and emotions into simple, shareable formats that facilitate rapid spread and impact. Coined by Richard Dawkins, who conceptualized them as cultural analogs to genes, memes self-replicate, mutate, and respond to selective pressures \cite{Dawkins_1976}. As such, the online memetic landscape continually evolves with the rapid emergence of new memes and variations of existing ones. By tapping into shared cultural references and experiences, memes use relatability to spread faster and use background knowledge to convey messages more succinctly \cite{Tommasinietal2023}. In the digital sphere, memes often manifest as variants of a particular image, video, or cliche disseminated by many users \cite{Zannettou.et.al.2018}.  Although memes can take various forms, they are most commonly recognized as static images often overlaid with text \cite{Onielfa.et.al.2022}, which is the primary focus of this study.

% Once a niche aspect of online communities like 4chan and Reddit, memes have surged in popularity due to the rise of social media and advancements in image-editing software, enabling amateurs and professionals alike to create and disseminate such content \cite{theisen.et.al.2020}. Memes can, therefore, be viewed as a mirror reflecting cultural and social trends; by studying them, we can derive valuable insights into the values, beliefs, and concerns of various communities and societies~\cite{shifman2019internet}. The proliferation of memes online has also led to potential dangers, further emphasizing the need for research in this area. Initially intended for humor or irony, memes are increasingly being used for malicious purposes, including targeted attacks on individuals, groups, and businesses, as well as coordinated hate campaigns \cite{Pramanick.et.al.2021,qu.et.al.2023}. Moreover, political actors have recognized the power of memes to influence societal beliefs and actions, leading to their use in spreading political messaging \cite{beskow.et.al.2020}. 


Once niche to communities like 4chan and Reddit, internet memes have gained widespread popularity due to social media and advancements in image-editing software \cite{theisen.et.al.2020}. 
Memes condense complex ideas into shareable formats, typically using text overlaid on images \cite{Onielfa.et.al.2022}, reflecting cultural and social trends \cite{shifman2019internet}. They express humor and irony but can also serve malicious purposes, such as coordinated hate campaigns and political messaging \cite{Pramanick.et.al.2021,qu.et.al.2023,beskow.et.al.2020}. 



\begin{figure}[!t]
    \begin{subfigure}[b]{0.25\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/original.jpg}
        \caption{Original}
        \label{fig:example_original}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.15\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/form.png}
        \caption{Form}
        \label{fig:example_form}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.15\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/visual_content.png}
        \caption{Visual Content}
        \label{fig:example_vcontent}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.15\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/textual_content.png}
        \caption{Textual Content}
        \label{fig:example_tcontent}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.15\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/identity.jpg}
        \caption{Identity}
        \label{fig:example_identity}
    \end{subfigure}
    \hfill
    % \begin{subfigure}[b]{0.15\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/stance.jpg}
    %     \caption{Stance}
    %     \label{fig:example_stance}
    % \end{subfigure}
    % \hfill
    \caption{The original ``Stonks'' meme template, accompanied by example memes related through various dimensions: form, visual and textual content, and identity.}
    \label{fig:examples_stonks}
\end{figure}

The rapid proliferation and diversity of memes online necessitate automated analysis. Yet, their subtle, multimodal nature \textemdash combining text, images, background knowledge, and context \textemdash makes this an AI-complete challenge. Research on internet memes deals with modeling how memes evolve and propagate across online communities \cite{Zannettou.et.al.2018,beskow.et.al.2020,qu.et.al.2023,Weng.et.al.2014}, analyzing the layered semantics and cultural contexts of memes \cite{Dancygier.Vandelanotte.2017,hee.et.al.2023}, applying machine learning to downstream learning tasks such as identifying hateful memes \cite{kiela2021hateful,thakur2023multimodal,Grasso-et-al-2024}, and developing methods to generate novel memes \cite{perison.tolunay.2018,wang-wen-2015-cheezburger}. 
%
% Problem statement
% We are solving three problems: 1.reliance on a knowledge base (of template approaches), 2. lack of consideration of semantics (of clustering approaches), and 3. lack of customization for different similarity dimensions (of all prior approaches).
Analytical tasks over memes necessitate a robust estimation of meme similarity and cluster discovery \cite{dubey.et.al.2018,theisen.et.al.2020}.
% Meme clustering is the core of such analytical tasks, which include virality modeling, toxicity identification, and cultural analysis.
% The consideration of meme similarity is at the core of the wide range of such tasks and methods. When are two memes sufficiently similar for one to be considered an adaptation of the other?
Standard bottom-up clustering methods~\cite{qu.et.al.2023,Zannettou.et.al.2018} are based on pixel-level similarity captured through either local or global features, which offer complementary strengths~\cite{theisen.2022}. Recognizing that such methods \textit{cannot capture memes' multi-dimensional and rich semantics}, another line of work grounds new memes to a knowledge repository of novel templates~\cite{joshi.et.al.2023,bates-et-al-2023}. Yet, \textit{existing template-based approaches rely on two strong assumptions: comprehensive database coverage and a single, form-driven similarity}. 


A more fundamental challenge with all existing methods is the lack of agreement on how memes should be grouped, i.e., what it means for two memes to be similar.
Real-world memes \textit{defy strict template boundaries and exhibit partial similarity}~\cite{pandiani2024toxic}. 
New variants continually emerge, borrowing elements from other memes, mimicking, remixing by superimposing new elements, or even repurposing images entirely, which makes their clustering relative to the dimension of interest.
Figure \ref{fig:examples_stonks} illustrates the ``Stonks'' meme (a) alongside related memes:\footnote{\url{https://knowyourmeme.com/memes/stonks}} a remix of the original template, keeping only its \textbf{form} with new superimposed visual and text elements (Figure \ref{fig:example_form}); a mimetic variation, retaining the \textbf{visual content} of a person in suit observing rising stock values but substituting the subject with another well-known meme personality (Figure \ref{fig:example_vcontent}); a variation of a different meme template\footnote{https://knowyourmeme.com/memes/steven-crowders-change-my-mind-campus-sign} related through \textbf{text} by appropriating the ``Stonks'' catchword; and an \textbf{identity} similarity case that features the same fictional entity (``Meme Man") also in an entirely different meme. These examples highlight the inherent challenges of matching these memes and defining what makes a coherent cluster. For instance, Figure \ref{fig:example_tcontent} could be grouped with the ``Stonks'' meme, other memes that follow the Steven Crowder campus sign format, or both. Figure \ref{fig:example_identity} raises the question whether character continuity alone constitutes sufficient grounds for grouping. As prior work does not consider clustering relative to the similarity dimensions of interest, we note a gap between assumptions in the literature and real-world memes.
In summary, we note three challenges with prior work: the lack of consideration of semantics (bottom-up clustering methods), the reliance on databases (template-based methods), and the lack of customization for similarity dimensions (all methods).









% RQ and contributions
% Our contributions then are threefold: we are proposing a more comprehensive method (that solves the issues 1 and 2), providing a way to connect similarity to feature sets (thus solving issue 3), and we provide a corresponding experimental analysis to validate our solutions to 1-3.

% In this paper, we investigate 
\textit{How can we develop a comprehensive and modular meme clustering method that can natively adapt to similarity dimensions (without a knowledge base of templates)?} Our contributions are:
\begin{enumerate*}
    \item \textbf{A comprehensive method for meme clustering}, which consolidates popular global and local feature extractors, enables clustering by identifying templates, and performs incremental meme matching to templates.
    \item \textbf{A modular approach to meme clustering}, which groups features into four similarity dimensions: form, visual content, text, and identity, and retrieves memes relative to a user-defined dimension.
    % . We dynamically retrieve memes based on the most relevant aspects of their meaning and content relative to a similarity dimension of interest.
    \item \textbf{Extensive experiments} with existing data and human validation to evaluate the impact of using a comprehensive set of features and the alignment between similarity features and task dimensions. Our experiments show that a more comprehensive framework leads to superior performance, whereas aligning features to dimensions allows flexible matching for a similarity dimension.
\end{enumerate*}






% This study aims to cluster memes in a way that systemically addresses these various considerations. Specifically, we propose a novel approach that constructs rich feature representations to identify and group similar memes across various dimensions, including form, visual and textual content, and identity. To avoid assumptions about which aspects of meme similarity to prioritize, we dynamically retrieve memes based on the most relevant aspects of their meaning and content about a user query. To achieve this, we extract a selection of both global and local features from memes and cluster using a two-step process: first, we identify templates using stringent clustering methods; then, we incrementally match memes to these templates based on the feature set that best represents the desired aspect of similarity. 


% We validate our method by comparing it to conventional approaches where clustering is directly applied to the graph, utilizing human feedback to review clusters, and assessing its alignment with curated meme databases such as KnowYourMeme. Our findings indicate that both the combination of features and the matching to templates contribute to more meaningful clusters compared to conventional methods.  We validate that the features effectively capture the intended aspects of meme similarity and show how much they can reliably match memes to the identified templates. Additionally, we developed a user interface to demonstrate, using various examples, how our method can be applied in a downstream application that dynamically retrieves the most relevant memes.

